To what extent homophily and influencer networks explain song popularity

Forecasting the popularity of new songs has become a standard practice in the music industry and provides a comparative advantage for those that do it well. Considerable efforts were put into machine learning prediction models for that purpose. It is known that in these models, relevant predictive parameters include intrinsic lyrical and acoustic characteristics, extrinsic factors (e.g., publisher influence and support), and the previous popularity of the artists. Much less attention was given to the social components of the spreading of song popularity. Recently, evidence for musical homophily - the tendency that people who are socially linked also share musical tastes - was reported. Here we determine how musical homophily can be used to predict song popularity. The study is based on an extensive dataset from the last.fm online music platform from which we can extract social links between listeners and their listening patterns. To quantify the importance of networks in the spreading of songs that eventually determines their popularity, we use musical homophily to design a predictive influence parameter and show that its inclusion in state-of-the-art machine learning models enhances predictions of song popularity. The influence parameter improves the prediction precision (TP/(TP+FN)) by about 50% from 0.14 to 0.21, indicating that the social component in the spreading of music plays at least as significant a role as the artist's popularity or the impact of the genre.

==> notes.tex <==
% [================ Literature about predicting song success ======================]

% I summarized the most relevant literature here for reference

% \cite{Pachet_2008}
% In 2008: Hit song science is not yet a science - they show that at that time, machine learning was not suitable for predicting the popularity of songs.

% \cite{Pachet_2012}
% About the field of hit song science

% \cite{Interiano_2018}
% Songs in UK between 1985 and 2015. They define success as making it into the charts. They correlate success with acoustic features which they got from musicbrainz. They find that successful songs are "happier" more "party-like" and more "female". In general, they find a trend that music became less "happy" and more "sad" but also more "danceable" over time.

% Influence of labels and position on an album on the survivability of a song
% https://www.sciencedirect.com/science/article/pii/S0736585317305695?casa_token=vf2L8SzVGcsAAAAA:wgSQdurmGjjEug3W8IwXySk3BPaMsBOEIt5GNyewLFHMfkgHepF93jzxwv0asd67Cl3aTnVsIoA
% \cite{Hyunsuk_2018}
% Survival analysis. They look at the top 100 charts of Korea. looking at streaming and download (digital market). try to find factors that influence how long songs 'survive' in the charts. Most important factor: being the title track. Then: major labels have more downloads. Songs of superstar artists survive longer. Tie-ins (connections with other media, e.g. being on the title track of a movie) have a negative effect. They might help in reaching the charts, but they have a higher chance to drop from them again. They mention the 'bandwagon effect' = preferential attachment.

% SVM success prediction of artists
% https://dl.acm.org/doi/abs/10.1145/3330482.3330493?casa_token=Nmn4ZJo9O94AAAAA:dbJaV7uzifX0z8q_EWgCygc6M9slBaaFs1rp0XAxx2P0TcDkpQhpZLoF3K8uauRD50T0Ju2QRXZNxg
% \cite{Yu_2019}
% SVM and neural network to predict the popularity of songs. On a dataset collected by the Alibaba group in China during a competition. They train on 4 months of data and then try to predict the daily listenings per song for the next 2 months. They are only using the play history and download history, no other data. Results: it's challenging. more features improve the prediction. SVm performs a little better than neural network.

% Success prediction using lyric and acoustic features
% https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.86.4054&rep=rep1&type=pdf
% \cite{Dhanaraj_2005}
% They try to identify potential hit songs. They use SVM and boost classifiers, input are lyrics and acoustic features. They find that the prediction is much better than random, with lyrical features performing a bit better than acoustic features. Combining both does not improve over taking only one.

% Relates repetition in lyrics to success
% https://www.narcis.nl/publication/RecordID/oai:pure.knaw.nl:publications%2F4a56b6f6-4e6c-4757-a28e-010e8c6b8d28
% \cite{Lassche_2019}
% Study the textual repetition in songs. They find that songs have a greater chance of becoming popular if the lyrics are more repetitive.

% success dynamics
% https://doi.org/10.1142/S021952591850008X
% \cite{Shin_2018}
% They look at on-chart life-trajectories of songs i.e. when songs enter charts, how long they stay there and when they exit them. They characterize these life-trajectories. They study a dataset of 7000 Korean pop songs. They find that there is a strong influence of non-musical factors such as the established fan-base of the artist and the influence of the production company.

% https://link.springer.com/chapter/10.1007/978-3-030-49161-1_6
% predicting song success based on sentiment analysis on twitter
% \cite{Tsiara_2020}
% They look at the top 100 charts. They check on Twitter how often a song and an artist are mentioned as well as the sentiment of the tweets. They do a regression and try to predict how the chart positions are changing. They find a moderate correlation between the count of \#nowplaying of a song and the chart position as well as a weak correlation between the sentiment of the tweets and the chart position.

% https://www.sciencedirect.com/science/article/pii/S0167923621000452?casa_token=pl0GIjpmIUsAAAAA:f5pwLqvPF4wE_1_jx3yIeIPcSWsoJCwKB9j1dYYktVGE1IK2TrpnFTO8wmzzERZ1Fu_DCHyW_OU
% using acoustic features to predict success
% \cite{Kim_2021}
% Superstars significantly dominate the market share. They use acoustic features from spotify such as danceability, happiness to predict the chart position of songs. They do a regression. They find that happier, more danceable songs are more likely to be a hit song. They also find a correlation with the number of songs an artist has released.

% https://journals.sagepub.com/doi/full/10.1177/0003122417728662?casa_token=LRfW_wImxwwAAAAA%3A-6EPhCPrb8BD2wsuN2rWg4yGeNsQ-xVofVupYkx9i0rUOC6rDTvVYnv03mWCKqC0dG5d9-BOaw9RIw
% what makes pop music popular
% \cite{Askin_2017}
% They ask what makes a pop song popular. They try to predict the success of chart songs (their chart position) based on their features. They find that popularity of the artist, support of the publisher, the genre have an impact. They also find that songs sounding too similar to other songs are less likely to succeed. They argue that there is a sweet spot of differentiation.

% https://royalsocietypublishing.org/doi/full/10.1098/rspa.2021.0457
% modelling song spreading like infectious disease spreading
% \cite{Rosati_2021}
% They look at song downloads on mobile phones. They use a SIR disease spreading model to model the downloads of songs. They argue that social processes that lead to the spread of music are similar to disease spreading. They find that in some genres the connectivity is higher and songs spread faster. 

% http://cs229.stanford.edu/proj2015/140_report.pdf
% predict song success based on audio features and metadata
% \cite{Pham_2016}
% They use the million song dataset and use audio features and metadata to predict the success of songs. They find that the metadata is much more predictive than the audio features. The most predictive features they find are: artist familiarity, loudness, year, number of genre tags

% https://arxiv.org/abs/1908.08609
% hit song prediction with spotify data
% \cite{Middlebrook_2019}
% Attempting to solve the hit song science problem: which songs will become chart hits. They look at 1.8 million songs on spotify and extract their audio features. They use logistic regression, neural network, svm and random forest. Random forest performed best. They reached 88\% accuracy (with balanced groups).

% https://dl.acm.org/doi/abs/10.1145/2632188.2632206?casa_token=rrTFe2gsqX0AAAAA:0fCXB7LKr__hyPgJ1I2Wf0Vg26ugcC7HetrJQzvRc7Bphhz4foGyWqAF-h23BmfdUoh11tZkVLporQ
% twitter for prediction
% \cite{Kim_2014}
% They look at Twitter and look for music related hashtags such as \#nowplaying. They use these hashtags in a predictive model and predict the chart rankings of songs. They find that the number of daily tweets about a specific song and artist is highly correlated with the general trend of that song.


% deep learning on the audio features to predict hits
% \cite{Yang_2017}
% They build a convolutional neural network and use it to learn how the audio features of songs influence the popularity of Chinese and western pop songs in Taiwan. They confirm that deep structures are superior to shallow structures in capturing the audio features of songs.


% Hit song science
% \cite{Ni_2011}
% They argue that predicting the popularity of songs is feasibly given a relevant set of acoustic song features. They demonstrate this with a machine learning approach.



% check references of references


% === Other relevant literature that is not concerned with predictions ====

% homophily
% https://www.jstor.org/stable/2678628
% Similarity breeds connection. people's personal networks are homogeneous with regard to many sociodemographic, behavioral, and intrapersonal characteristics. Homophily limits people's social worlds in a way that has powerful implications for the information they receive, the attitudes they form, and the interactions they experience.

% Prediction based on online searches
% https://www.pnas.org/doi/abs/10.1073/pnas.1005962107
% They find that online search trends are highly predictive of song charts.

% predicting friendship links in lastfm (result: taste alone rarely leads to friendships. mostly it's having friends together that leads to friends.)
% https://dl.acm.org/doi/abs/10.1145/2380718.2380725?casa_token=XWlKVK_QMRoAAAAA:km0zNBZwbkVd87ZfdzUBQBL4v23MwSoxzPoJv_DXYgDe_0L1tUHYR-5nVL1417RrqJn-907hhTxKMg
\cite{10.1145/2380718.2380725}

% lastfm social network recommendations
% https://doi.org/10.1007/s13278-014-0244-y
% https://arxiv.org/abs/1307.7142
% Information about new artists spreads through social links. There is homophily friends. They define a an influence measure. They use it to improve song recommendations for users. They build a recommendation system: If a close friend listens to a song, the user is recommended that song. 
\cite{P_lovics_2015}

% Lastfm - do friends listen to the same music?
% https://link.springer.com/chapter/10.1007/978-3-030-54994-7_11
% They build a model for each user of what they listen to and their listening behaviour. They find that similar users cluster together in the friendship network, but similarity in music taste does not increase the probability of people to become friends.
\cite{10.1007/978-3-030-54994-7_11}

% Qualitative interviews about lastfm usage
% https://www.inderscienceonline.com/doi/abs/10.1504/IJWBC.2011.039513
% user-to-user communication is often limited to users that already know each other in person (Anchored relationships). People use lastfm to find music they like based on what they liked before. 
\cite{doi:10.1504/IJWBC.2011.039513}

% homophily in music
% https://dl.acm.org/doi/abs/10.1145/3487351.3492706
% they study homophily on last.fm
% they compute user- artist profiles 
% users that are friends share similar music taste
% diversity of music helps to predict friendships. especially high novelty seekers (explorers) show strong homophily (like vittorios paper)
% they predict friendship links based on that

% Social interactions affect discovery processes
% https://doi.org/10.48550/arXiv.2202.05099
% Users on last.fm. There are heterogeneous discovery rates. User behaviour is influenced by their friends. especially highly explorative users tend to be friends with users that have similar discovery rates.
\cite{DiBona_2022}

% music plays a role in how we choose friends
% https://www.ncbi.nlm.nih.gov/pmc/articles/PMC5491604/
% Music is a highly significant and meaningful medium, particularly in adolescence
%  for identity and social identity development
%  indicated that adolescents select their friends based on both externalizing behavior and highbrow music preference




% model & prediction category &  \\
% \hline
% (a) combined model    & accuracy &         \textbf{0.98} & $ 10^{-5}$  \\
%     & hit-precision &     \textbf{0.21} & 0.0 \\
%     & non-hit precision & 1.0 & 0.0  \\
%     & hit recall &        \textbf{0.60} & 0.006 \\
%     & non-hit recall &    \textbf{0.99} & $ 10^{-5}$  \\
% \hline
% % & & & var \\
% (b) social network only    & accuracy &         0.95 & $ 10^{-5}$  \\
%     & hit-precision &     0.05 & 0.0  \\
%     & non-hit precision & 1.0 & 0.0  \\
%     & hit recall &        0.40 & 0.004 \\
%     & non-hit recall &    0.96 & $ 10^{-5}$  \\
% \hline
% % & & & var \\
% (c) without social network    & accuracy &         \textbf{0.97} & $ 10^{-5}$  \\
%     & hit-precision &     \textbf{0.14} & 0.0  \\
%     & non-hit precision & 1.0 & 0.0  \\
%     & hit recall &        \textbf{0.70} & 0.005  \\
%     & non-hit recall &    \textbf{0.98} & $ 10^{-5}$ \\

